LFOC+: A Fair OS-level Cache-Clustering Policy for Commodity Multicore Systems

Commodity multicore systems are increasingly adopting hardware support that enables the system software to partition the last-level cache (LLC). This support makes it possible for the operating system (OS) or the Virtual Machine Monitor (VMM) to mitigate shared-resource contention effects on multicores by assigning different co-running applications to various cache partitions. Recently cache-clustering (or partition-sharing) strategies have emerged as a way to improve system throughput and fairness on new platforms with cache-partitioning support. As opposed to strict cache-partitioning, which allocates separate cache partitions to each application, cache-clustering allows partitions to be shared by a group of applications. In this article we propose LFOC+, a fairness-aware OS-level cache-clustering policy for commodity multicore systems. LFOC+ tries to mimic the behavior of the optimal cache-clustering solution for fairness, which we could obtain for different workload scenarios by using a simulation tool. Our dynamic cache-clustering strategy continuously gathers data from performance monitoring counters to classify applications at runtime based on the degree of cache sensitivity and contentiousness, and effectively separates cache-sensitive applications from aggressor programs to improve fairness, while providing acceptable system throughput. We implemented LFOC+ in the Linux kernel and evaluated it on a real system featuring an Intel Skylake processor, where we compare its effectiveness to that of four previously proposed cache-clustering policies. Our experimental analysis reveals that LFOC+ constitutes a lightweight OS-level policy and improves fairness relative to two other state-of-the-art fairness-aware strategies --Dunn and LFOC--, by up to 22\% and up to 20.6\%, respectively, and by 9\% and 4.9\% on average.

==> Makefile <==
DOCS = main
ALLTEXFILES = $(wildcard *.tex)
TEXFILES = $(patsubst %,%.tex,$(DOCS))
DVIFILES = $(patsubst %,%.dvi,$(DOCS))
PSFILES = $(patsubst %,%.ps,$(DOCS))
PDFFILES = $(patsubst %,%.pdf,$(DOCS))
TEXCODE = 
#$(patsubst code/%.c, code/%.tex, $(wildcard code/*.c))

#all: $(TEXCODE) $(DVIFILES) $(PSFILES) $(PDFFILES)
all: $(DVIFILES) $(PSFILES) $(PDFFILES)

%.dvi: $(ALLTEXFILES)
	latex $*
	bibtex $*
	latex $*
	latex $*

%.ps: %.dvi
	dvips  -X 1200 -Y 1200 $< -o $@

%.pdf: %.ps
#	lpr -P APDF $<
#	sleep 5
#	mv $(HOME)/PDF/$@ .
	ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true $<

wc: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  wc $$tex; \
	done;

spellcheck: $(TEXFILES)
	@for tex in $(TEXFILES); do \
	  ispell -t -d american $$tex; \
	done;	

clean:
	@rm -f *.out *.bbl *.blg *.dvi *~ *.ps *.aux *.log *.pdf code/*.tex code/*~ *.bak



